Hardware-Assisted Detection of Firmware Attacks in Inverter-Based Cyberphysical Microgrids

The electric grid modernization effort relies on the extensive deployment of microgrid (MG) systems. MGs integrate renewable resources and energy storage systems, allowing to generate economic and zero-carbon footprint electricity, deliver sustainable energy to communities using local energy resources, and enhance grid resilience. MGs as cyberphysical systems include interconnected devices that measure, control, and actuate energy resources and loads. For optimal operation, cyberphysical MGs regulate the onsite energy generation through support functions enabled by smart inverters. Smart inverters, being consumer electronic firmware-based devices, are susceptible to increasing security threats. If inverters are maliciously controlled, they can significantly disrupt MG operation and electricity delivery as well as impact the grid stability. In this paper, we demonstrate the impact of denial-of-service (DoS) as well as controller and setpoint modification attacks on a simulated MG system. Furthermore, we employ custom-built hardware performance counters (HPCs) as design-for-security (DfS) primitives to detect malicious firmware modifications on MG inverters. The proposed HPCs measure periodically the order of various instruction types within the MG inverter's firmware code. Our experiments illustrate that the firmware modifications are successfully identified by our custom-built HPCs utilizing various machine learning-based classifiers.

==> Sections/Review.tex <==
\begingroup
\let\clearpage\relax 
\onecolumn 

%\setstretch{2}

\fontfamily{bch}\selectfont 

\null\vspace{2cm}
\noindent Dear Associate Editor and Reviewers,\\ 

\noindent We appreciate your positive comments on our work and we would like to
thank you for the valuable feedback about our submission to the \textit{International Journal of Electrical Power and Energy Systems}.
Please find an updated version of our manuscript that has been
accordingly revised.\\

\noindent The main changes to the revised manuscript are as follows: 
\begin{itemize}
\item We have provided a thorough explanation and analysis on the power and area overhead of our HPC design;
\item We have included discussion on the feasibility of our method for potential implementations in prevalent architectures;
\item We have revised the manuscript to remove redundancies, fix grammar mistakes, improve figure aesthetics, and create consistent references;
\item We have included detailed clarifications on the false positive and negatives furnished by our proposed technique.\\
\end{itemize}
 
\noindent Our complete and detailed comments on your specific points appear
below in {\em italics}. We have addressed all the issues in the
revised manuscript.\\

\noindent 
%All modifications performed on the manuscript are highlighted in {\color{red} red color}.
 
~\newline
Best regards,

\noindent 
Abraham Peedikayil Kuruvila, Ioannis Zografopoulos, Kanad Basu, and Charalambos Konstantinou

\newpage

%\setstretch{1.1}


\begin{center}
\large {\bf Reviewer 1}
\end{center}

\noindent{\bf Q-R1.1: From my understanding, the implemented in hardware ML classifiers have the purpose just to demonstrate the approach's area and power overhead if actually existed in inverters. If this is the case, are those cell libraries the ones used in power grid controllers? How was this selection done? Also, please elaborate on Table I results: is such overhead reasonable for low-end embedded systems like microinverters?
}

\vspace{4pt}
\noindent{\em {\bf A-R1.1:} We thank the reviewer for the excellent question.
\vspace{4pt}

`` We realized the machine learning classifiers in Figure~\ref{fig:HPC2chart} in hardware to determine their area and power overhead. We designed the Register Transfer Level (RTL) for the Decision Tree, Neural Network, and Random Forest classifiers and synthesized them through the Synopsys Design Compiler logic synthesis tool. We employed two digital standard cell libraries, lsi\_10k and saed\_90nm, as we had access to them for our synthesis tool. While other libraries could have been employed, the furnished power and area overhead numbers would be consistent with the values obtained from our existing libraries. The overhead results from Table~\ref{tab:my-table1} are reasonable expenditures for low-end embedded systems, as the power required is in the micro-watt range. Furthermore, we implemented our proposed custom-built HPCs into a simple MIPS processor using Xilinx Vivado High-Level Synthesis (HLS), which enables C to RTL conversion, to synthesize it for an Artix-7 FPGA. The MIPS processor was chosen as it is open source and incurs less area than other processors, such as Intel or ARM. Hence, the area overhead for our custom-built HPC design units would be lower in an Intel or ARM processor than in MIPS. Our custom-built HPC logic was added to the decode unit of the MIPS processor, and we incurred a maximum area overhead of 1.2\% in terms of LUTs. Consequently, implementing our custom-built HPCs into an ARM or Intel processor would result in less overhead. Therefore, low-end embedded systems would not incur much overhead incorporating our proposed methodology.

Additionally, both the area and the power consumption overheads stated in Table~\ref{tab:my-table1} should be regarded as essential additions for future inverter-based microgrid controllers for two main reasons. First, since inverters are part of the critical infrastructure, the security objective of their underlined embedded systems is of utmost importance. Even our worst-case scenario power consumption overheads range from few $\mu$W to tenths of mWs. Such small power tradeoffs are acceptable to enhance device security, and microinverter controllers are not considered low-power nor battery-operated embedded systems~\cite{10.1145/996566.996771}. Second, although the specific area and power consumption of the microinverter are not openly available (by the manufacturer) for direct comparisons, the proposed overheads can be compared against similar  microcontroller unit designs. Namely, the open core OpenMSP430 design layout discussed in \cite{PauloJoaoTemoteoRito_6_2018}, considers an embedded system occupying area of 1050x2800$\mu$m while consuming 1.99mW of power. On the other hand, the authors in~\cite{yang2020pcb} present a DC-AC inverter module occupying a vast printed circuit board (PCB) area of 90×40mm. The reported design specifications render our 1.2\% overhead totally insignificant, and a reasonable sacrifice for a more secure device. "

\textbf{We have included this discussion in Section~\ref{results-hardware}}
}

\vspace{14pt}
\noindent{\bf Q-R1.2: An added table would be beneficial to show the 30-n HPC-based feature vector utilized for the HPC-aware firmware modification detection.}

\vspace{4pt}
\noindent{\em {\bf A-R1.2:} We thank the reviewer for the useful suggestion. We have incorporated the HPC-based feature vector into a table to ensure clarity as shown in Table~\ref{featuretable-2}. The top row contains the custom-built HPCs relating to arithmetic, boolean, load, store, and branch/jump instructions as well as the various HPC combinations for the arithmetic instruction. The following rows show the different custom-built HPC combinations for the boolean, load, store, and branch/jump instructions.

\textbf{This table has been added to Section~\ref{sec:backgroundcustomHPCcollection}.}

%\begin{table*}[ht!]
%\centering
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%\multicolumn{6}{|c|}{\textbf{Feature Vector}} \\ \hline
%a     & aa    & ab    & al    & as    & an    \\ \hline
%b     & bb    & ba    & bl    & bs    & bn    \\ \hline
%l     & ll    & la    & lb    & ls    & ln    \\ \hline
%s     & ss    & sa    & sb    & sl    & sn    \\ \hline
%n     & nn    & na    & nb    & nl    & ns    \\ \hline
%\end{tabular}
%\caption{}
%\label{featuretable}
%\end{table*}






%\begin{table*}[ht!]
%\centering
%\caption{Proposed Custom-built HPCs.}
%\begin{tabular}{|c|c|c|c|c|}
%\hline
%\multicolumn{5}{|c|}{\textbf{Feature Vector}} \\ \hline
%a       & b       & l       & n      & s      \\ \hline
%aa      & bb      & ll      & nn     & ss     \\ \hline
%ab      & ba      & la      & na     & sa     \\ \hline
%al      & bl      & lb      & nb     & sb     \\ \hline
%an      & bn      & ln      & nl     & sl     \\ \hline
%\multicolumn{1}{|l|}{as} & \multicolumn{1}{l|}{bs} & \multicolumn{1}{l|}{ls} & %\multicolumn{1}{l|}{ns} & \multicolumn{1}{l|}{sn} \\ \hline
%\end{tabular}
%\label{featuretable-2}
%\end{table*}



\begin{table*}[ht!]
\centering
\caption{Proposed custom-built HPCs.}
\vspace{0.1in}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{10}{|c|}{\textbf{Feature Vector}}  \\ \hline
a  & b  & l  & n  & s  & aa & ab & al & an & as \\ \hline
bb & ba & bl & bn & bs & ll & la & lb & ln & ls \\ \hline
nn & na & nb & nl & ns & ss & sa & sb & sl & sn \\ \hline
\end{tabular}
\label{featuretable-2}
\end{table*}



}

\vspace{64pt}
\noindent{\bf Q-R1.3: Minor grammar errors and repetition exist throughout the text, and proof-reading carefully can help fix those.}

\vspace{4pt}
\noindent{\em {\bf A-R1.3:} \textcolor{black}{We thank the reviewer for the valuable feedback. We have thoroughly revised the manuscript to correct grammar mistakes and remove repetitions.} 
}


\vspace{14pt}
\noindent{\bf Q-R1.4: General, it is not recommended to cite more than three references at the same location, all at once, unless there is a very compelling reason for it. From the technical reader’s view point, it is not desirable to direct the reader to too many articles in order to find a minor point. Citing many papers at one location implies that the authors could not better organise their material. If there is no survey paper, the authors can better organise these references. For example, organize them in groups of three, and then explain the reasons behind their design rationales, and point out the differences.}

\vspace{4pt}
\noindent{\em {\bf A-R1.4:} We thank the reviewer for this suggestion, and we have adjusted the manuscript accordingly. We have only kept the critical references in order to state our points. In absence of tutorial papers encompassing all the essential information, we have kept up to two references throughout the whole paper. As advised by the reviewers, this will improve the readability of our paper, avoid reader confusion, and improve the overall quality of our manuscript. 

Some of the eliminated references included redundant citations providing background information on microgrid inverters and Hardware-assisted Malware Detectors (HMDs). Removing them has not affected the technical integrity of or manuscript. On the other hand, it has helped remove repetitions. Once again, we thank the reviewers for allowing us to improve our work using their insightful comments.

}

\vspace{14pt}
\noindent{\bf Q-R1.5: The technical language used in the paper could be improved. I recommend that the authors carefully read the technical writing notes by Donald E. Knuth, Tracy Larrabee, and Paul M. Roberts (please see http://tex.loria.fr/typographie/mathwriting.pdf), and revise the whole article accordingly.}

\vspace{4pt}
\noindent{\em {\bf A-R1.5:} \textcolor{black}{We thank the reviewer for this excellent suggestion. We have edited the manuscript's technical language and have fixed grammar issues in order to improve the overall quality of the paper. }}  




\vspace{14pt}
\noindent{\bf Q-R1.6:  Figures are not positioned correctly. 
 }

\vspace{4pt}
\noindent{\em {\bf A-R1.6:} We greatly appreciate the reviewer for their comment about the appearance of the paper. We have carefully revised the figures to improve their aesthetics and to appear on the same page they are referenced or the following one (if appearing on the same page was not possible). 
}



\newpage


\vspace{14pt}
\begin{center}
\large {\bf Reviewer 2}
\end{center}

\noindent{\bf Q-R2.1: References need consistency. Some include "et al." (not necessary) and some others (with a lot of authors) do not.  }

\vspace{4pt}
\noindent{\em {\bf A-R2.1:} We thank the reviewer for the comment, and per your insightful suggestion we have included all the authors of the referenced publications. 

}


\vspace{14pt}
\noindent{\bf Q-R2.2: Figs. 10-13 need to specify that y-axis is percentage.}

\vspace{4pt}
\noindent{\em {\bf A-R2.2}: We thank the reviewer for the excellent observation. Figures 10 through 13 have been revised, and their y-axes have been updated to indicate the percentage signs. }


\vspace{14pt}
\noindent{\bf Q-R2.3: Please revise the grammar of the abstract+entire manuscript for the final version. There are some sections that have a few grammatical errors.}

\vspace{4pt}
\noindent{\em {\bf A-R2.3}: We thank the reviewer for the comment. The manuscript has been reviewed to remove grammatical and syntax errors, repetitions, and other redundant information.  }

\newpage


\vspace{14pt}
\begin{center}
\large {\bf Reviewer 3}
\end{center}

\noindent{\bf Q-R3.1: While the choice of hardware performance counters for malicious behavior is a well established approach, the number of introduced HPCs seems excessive for the functionality they provide. A combination of a few HPCs (one for every considered instruction type) and a simple finite state machine that offers a short instruction transition memory (such as a typical branch predictor) could severely limit the introduced hardware overhead. While the addition of HPCs in future controller iterations seems feasible, the growing prevalence of hardware agnostic software that emulate controller function can render highly tailored hardware controllers obsolete. A short section which can propose a potential implementation on typical ARM architectures can add to the real-world feasibility of this approach. Introducing HPCs on ARM architectures to substantially increase the number of features of potential machine-learning algorithms is a popular topic in the embedded systems security community. }

\vspace{4pt}
\noindent{\em {\bf A-R3.1:} We thank the reviewer for the comment. 
\vspace{4pt}

`` We do not have access to an open source ARM architectural implementation. As a result, in order to assess the hardware overhead of custom-built HPCs, we implemented them into a simple MIPS processor using Xilinx Vivado High-Level Synthesis (HLS), which enables a C to Register Transfer Level (RTL) conversion, and synthesized it for an Artix-7 FPGA. The MIPS processor was chosen as it is open source and incurs less area overhead than an ARM or Intel processor. Hence, the area overhead for our custom-built HPC design units would be lower in an Intel or ARM processor than in MIPS. Therefore, the obtained results provide a pessimistic estimate for area overhead. Our custom-built HPC logic was added to the decode unit of the MIPS processor, and we incurred a maximum area overhead of 1.2\% in terms of LUTs, which is extremely insignificant. As a result, our custom-built HPCs implemented on an ARM or Intel processor would have considerably lower overhead. "

\textbf{This discussion has been added to Section~\ref{results-2}}.


}

\vspace{14pt}
\noindent{\bf Q-R3.2:  In the experimental section of the paper, the authors measure a synthetic output for overall accuracy which includes both false positive and false negative occurrences. However, based on the assumed criticality of a potential attack on microgrids, false negative instances can be much more damaging than false positives which could be overcome by a firmware update or replacement. What is the ratio of false positive vs false negative occurrences? In contrast, if the introduced scheme is a constant protection mode, like an antivirus, and a check is performed on a regular basis (e.g. every hour or so) false positives can negatively affect performance.}




\vspace{4pt}
\noindent{\em {\bf A-R3.2}: We thank the reviewer for this question. 
\vspace{4pt}

`` As shown in Figure~\ref{fig:HPC1chart}, all three of the utilized models were able to correctly identify most of the samples. However, there is only one golden custom-built HPC trace and four malicious attack traces. The imbalance of the dataset can lead to a biased ratio of false positives and false negatives. Consequently, we balanced the number of benign and malicious data and retrained our classifiers as shown in Figure~\ref{fig:revisionchart2} with the Random Forest furnishing 93.75\% accuracy, 91.66\% precision, and 95.65\% recall. Similar to before, all three of our classifiers correctly classified a majority of the data. Among the misclassified samples, the false positive to false negative percent ratios are: 15.7\% to 2.5\% for Decision Tree, 19.6\% to 7.5\% for Neural Network, and 8\% to 4.5\% for Random Forest.
%For the minority of misclassified samples, the false positive to false negative ratios are: 5 to 1 for Decision Tree, 11 to 2 for Neural Network, and 7 to 1 for Random Forest.
The low number of false negatives indicates the robustness of our proposed methodology in identifying the malicious inverter attacks. 

Additionally, when analyzing the effects of false positives negatively affecting performance, we consider two particular points. First, from Figure~\ref{fig:revisionchart2}, our proposed methodology is successfully able to identify 93.75\% of samples. Therefore, the number of false positives is relatively low, thereby leading to infrequent disruptions in inverter performance. Second, when ensuring system security for inverters, the minuscule amount of false positives is an acceptable trade-off for identifying nearly all malicious samples. As a result, when considering the strengthened security obtained and the infrequent negative effects on performance, our proposed methodology provides a robust defense."

\textbf{This discussion has been added to Section~\ref{results-1}}.



%\vspace{2mm}
\begin{figure}[!t]
\centering
  \includegraphics[width=0.9\linewidth]{Figures/revision-chart-1-2.pdf}
  %\vspace{-0.05in}
  \caption{Malicious firmware detection analysis with balanced dataset.}
  %\vspace{-2mm}
  \label{fig:revisionchart2}
  %\vspace{-0.05in}
\end{figure}


}


\endgroup

